Zef: Low-latency, Scalable, Private Payments

We introduce Zef, the first Byzantine-Fault Tolerant (BFT) protocol to support payments in anonymous digital coins at arbitrary scale. Zef follows the communication and security model of FastPay: both protocols are asynchronous, low-latency, linearly-scalable, and powered by partially-trusted sharded authorities. Zef further introduces opaque coins represented as off-chain certificates that are bound to user accounts. In order to hide the face values of coins when a payment operation consumes or creates them, Zef uses random commitments and NIZK proofs. Created coins are made unlinkable using the blind and randomizable threshold anonymous credentials of Coconut. To control storage costs associated with coin replay prevention, Zef accounts are designed so that data can be safely removed once an account is deactivated. Besides the specifications and a detailed analysis of the protocol, we are making available an open-source implementation of Zef in Rust. Our extensive benchmarks on AWS confirm textbook linear scalability and demonstrate a confirmation time under one second at nominal capacity. Compared to existing anonymous payment systems based on a blockchain, this represents a latency speedup of three orders of magnitude, with no theoretical limit on throughput.

==> Sections/construction.tex <==
\section{Coconut Construction} \label{sec:construction}

% \newcommand\alg[2]{\ding{118}\xspace \textsf{#1}\xspace$\bm{\rightarrow}$\xspace(#2):\xspace}

\subsection{Anon. credentials: Definitions}
\alberto{TODO}

\subsection{Coconut++: An example of anon. cred}
Objects (credentials) look like this: $\sigma = (h, s) = (h, h^{x+\sum_i m_i y_i}) \in \mathbb{G}_1$; 
the authorities secret keys are $(x, \{ y_i \})$, and their public keys are $(\alpha, \{ \beta_i \}) = (g_2^x, \{ g_2^{y_i} \}) \in \mathbb{G}_2$ and $\{ \gamma_i \} = g_1^{y_i} \in \mathbb{G}_1$.

\begin{description}[leftmargin=1em, labelindent=0em]
\setlength\itemsep{0.5em}

% Setup
\item[\alg{Setup($1^\lambda$)}{$params$}] Choose a bilinear group $(\mathbb{G}_1,\mathbb{G}_2,\mathbb{G}_T)$ with order $p$, where $p$ is a $\lambda$-bit prime number. Let $g_1, h_*$ be generators of $\mathbb{G}_1$, and $g_2$ a generator of $\mathbb{G}_2$. The system parameters are $params=(\mathbb{G}_1, \mathbb{G}_2, \mathbb{G}_T, p, g_1, g_2, h_*)$. 

% PrepareBlindSign
\item[\alg{PrepareBlindSign($\{m_i\}, \phi$)}{$\{k_i\},\Lambda,\phi$}]
The users picks a random $o\in\mathbb{F}_p$,  compute the commitment $c_m$ and the group element $h\in\mathbb{G}_1$ as follows:
\begin{equation}\nonumber
c_m = h_*^o \prod_i g_1^{m_i}  \qquad{\rm and}\qquad h = H(c_m)
\end{equation} 
Pick a random $\{k_i\} \in \mathbb{F}_p$ and compute the following commitments:
\begin{equation}\nonumber
\{c_i\} = \{ h^{m_i} g_1^{k_i} \} \qquad \forall m_i
\end{equation}
Output $(\{k_i\}, \Lambda=(c_m, \{c_i\}, \pi_{s}), \phi)$, where $\phi$ is an application-specific predicate satisfied by $\{m_i\}$, and $\pi_{s}$ is defined by:
\begin{equation} \nonumber
\pi_{s} = {\rm NIZK}\{(\{m_i\}, o, \{k_i\}): \{c_i\} = \{ h^{m_i} g_1^{k_i} \} \;\land\; c_m = h_*^o \prod_i g_1^{m_i} \;\land\;  \phi(\{m_i\})=1\}
\end{equation}

% BlindSign
\item[\alg{BlindSign($sk_j, \Lambda, \phi$)}{$\tilde{\sigma}_j$}] The authority $j$ parses $\Lambda=(c_m, \{c_i\}, \pi_{s})$, and $sk_j=(x_j, \{y_{(j,i)}\})$. Recompute $h = H(c_m)$. Verify the proof $\pi_{s}$ using $\{c_i\}, c_m$ and $\phi$; if the proof is valid, build $\tilde{c}_j = h^{x_j} \prod_i c_i^{y_{(j,i)}}$ and output $\tilde{\sigma}_j = (h, \tilde{c}_j)$; otherwise output $\perp$.

% Unblind
\item[\alg{Unblind($\tilde{\sigma}_j, \{k_i\}, \{ \gamma_i \}$)}{$\sigma_j$}] The users parse $\tilde{\sigma}_j=(h, \tilde{c})$; compute $\sigma_j = (h,\tilde{c} \prod_i \gamma_i^{-k_i})$. Output $\sigma_i$.

% AggCred
\item[\alg{AggCred($\{\sigma_j \}$)}{$\sigma$}] Parse each $\sigma_j$ as $(h,s_j)$. Output $(h,\prod^t_{j=1} s_j^{l_j})$, where $l$ is the Lagrange coefficient:
\begin{equation}\nonumber
l_j = \left[\prod^t_{k=1, k\neq j} (0-k)\right] \left[\prod^t_{k=1, k\neq j} (j-k)\right]^{-1} \;{\rm mod}\; p
\end{equation}

% ProveCred
\item[\alg{ProveCred($vk, \{ m_i \}, \sigma, \phi'$)}{$\Theta,\phi'$}]
Parse $\sigma=(h,s)$ and $vk=(g_2,\alpha,\{ \beta_i \})$. Pick at random $r',r \in \mathbb{F}_p^2$; set $h'=h^{r'}$, $s'=s^{r'} (h')^r$, and
$\sigma'=(h',s')$. Build $\kappa = \alpha g_2^r \prod_i \beta_i^{m_i}$. Output $(\Theta=(\kappa, \sigma',\pi_v),\phi')$, where $\phi'$ is an application-specific predicate satisfied by $\{ m_i \}$, and $\pi_v$ is:
\begin{equation}\nonumber
    \pi_v={\rm NIZK}\{(\{ m_i \},r): \kappa=\alpha g_2^r \prod_i \beta_i^{m_i} \ \land \  \phi'(\{ m_i \})=1\} 
\end{equation}

% VerifyCred
\item[\alg{VerifyCred($vk, \Theta, \phi'$)}{$true/false$}] Parse $\Theta = (\kappa, \sigma',\pi_v)$ and $\sigma'=(h',s')$; verify $\pi_v$ using $vk$ and $\phi'$. Output $true$ if the proof verifies, $h'\neq1$ and $e(h',\kappa)=e(s', g_2)$; otherwise output $false$.

\end{description}

\subsection{Protocol attempt}
Let's first try with the coin app. We use the scheme before with  three private attributes ($m_1$, $m_2$, $m_3$): the value of the coin, a random nonce, and the serialized public key of the recipient. A coin is a signature $\sigma$.

Let's call $\{v_i\}$ the value of the input coins (the ones we want to spend), and $\{w_i\}$ the value of the output coins (the ones we want to create). Let's call $\{s_j\}$ the nonce associated with input coins and $\{t_j\}$ the nonce associated with the output coins. 
%Let's call $p$ the serialized public key of the sender and $q$ the serialized public key of the recipient coins

\begin{description}[leftmargin=1em, labelindent=0em]
\setlength\itemsep{0.5em}

\item[Step0] Run a FastPay round as described in \Cref{sec:protocol}, that is get a certificate on a spent coin.

\item[\alg{Step1:Sender($vk, p, q, \{v_{i}\}, \{s_{i}\}, \{\sigma_{i}\}, \{w_{j}\}, \{t_{j}\}$)}{$m_M$}] \ \ \\
Compute $\{ \zeta_i = g_1^{s_i} \}$; 
pick at random $\{ o_i \}, \{ o'_j \} \leftarrow \mathbb{F}_p^{i+j}$; 
compute:
$$ \{ c_i = g_1^{v_i}h_*^{o_i} \} \quad ;  \{ d_j = g_1^{-w_j}h_*^{o'_j} \}$$
then compute:
\begin{eqnarray}\nonumber
&& \{ (\Theta_i, \phi') = \textsf{CO.ProveCred($vk, v_i, s_i, p \sigma_i, \phi'$)} \} \\ \nonumber
&& \{ (k, \Lambda_j, \phi') = \textsf{CO.PrepareBlindSign($w_i, t_i, q, \phi'$)} \}
\end{eqnarray}
where $\phi'$ is the statement:
\begin{eqnarray}\nonumber
&& \phi' = \{ 
\{\zeta_i = g_1^{s_i} \} \;\land\; 
\{ c_i = g_1^{v_i}h_*^{o_i} \} \;\land\; 
\{ d_i = g_1^{-w_i}h_*^{o'_i} \} \;\land\; 
\prod_i c_i \prod_j d_j = \prod_i h_*^{o_i} \prod_i h_*^{o'_i} 
\\ \nonumber
&& \quad \;\land\;  \{w_i \in [0,\mathit{MAX}] \}
\}
\end{eqnarray}
Broadcast to the authorities: $m_M = (\{\Theta_i\}, \{ \zeta_i \}, \phi', \{ c_i \}, \{d_j\}, \{\Lambda_j\})$.


\item[\alg{Step2:Authority($vk, m_M$)}{$\widetilde{\sigma}$}] \ \ \\
Parse the message $m_M = (\{\Theta_i\}, \{ \zeta_i \}, \phi', \{ c_i \}, \{d_j\}, \{\Lambda_j\})$. 
Output $\perp$ if any of $\{\zeta_i\} \in \mathcal{L}$; otherwise verify the proofs $\{\Theta_i$\}, and $\{\Lambda_j\}$ and the statement $\phi'$ running:
$$ \{ b = \textsf{CO.VerifyCred($vk, \Theta_i, \phi'$)} \}$$
and
$$ \{ \widetilde{\sigma} = \textsf{CO.BlindSign($vk, \Lambda_j, \phi'$)} \} $$
If all check pass, add all $\{ \zeta_i$ \} to the spent-list $\mathcal{L}$ and send back $\widetilde{\sigma}_i$ to the user.

\item[Step3.Sender:] Unblind $\widetilde{\sigma}$ and aggregate them into a single credential. Give $\{w_{j}\}, \{t_{j}\}$ to the recipient so that it can spend the new coins.

\item[Step4.Recipient:] Need to spend the coins now otherwise the Sender may steal them (it knows as much as the Recipient). \alberto{Can we add the recipient public key in the credential so that only the recipient can spend the new coin? } 
\end{description}

